xLAM: A Family of Large Action Models to Empower AI Agent Systems

Autonomous agents powered by large language models (LLMs) have attracted significant research interest. However, the open-source community faces many challenges in developing specialized models for agent tasks, driven by the scarcity of high-quality agent datasets and the absence of standard protocols in this area. We introduce and publicly release xLAM, a series of large action models designed for AI agent tasks. The xLAM series includes five models with both dense and mixture-of-expert architectures, ranging from 1B to 8x22B parameters, trained using a scalable, flexible pipeline that unifies, augments, and synthesizes diverse datasets to enhance AI agents' generalizability and performance across varied environments. Our experimental results demonstrate that xLAM consistently delivers exceptional performance across multiple agent ability benchmarks, notably securing the 1st position on the Berkeley Function-Calling Leaderboard, outperforming GPT-4, Claude-3, and many other models in terms of tool use. By releasing the xLAM series, we aim to advance the performance of open-source LLMs for autonomous AI agents, potentially accelerating progress and democratizing access to high-performance models for agent tasks. Models are available at https://huggingface.co/collections/Salesforce/xlam-models-65f00e2a0a63bbcd1c2dade4

==> 8-limitations.tex <==
\section{Limitations}




Our data synthesis pipeline relies on large LLMs such as DeepSeek-V2 and Mixtral-8x22b-Inst. This dependence may result in extended data generation times when utilizing less powerful GPUs.
Future work will focus on developing more efficient pipelines capable of operating effectively with both smaller and larger LLMs.

Additionally, due to the instability of some benchmarks and environments, along with the heavy reliance on API calls from commercial models such as OpenAI GPT-4, and constrained by limited research budgets, 
we face challenges in evaluating our models across even more benchmarks. Consequently, this may result in performance 
discrepancies on certain benchmarks. Moving forward, we aim to enhance our contributions to the research community by addressing instability and better maintaining and unifying existing benchmarks and environments.







